Towards Robust Direction Invariance in Character Animation

In character animation, direction invariance is a desirable property. That is, a pose facing north and the same pose facing south are considered the same; a character that can walk to the north is expected to be able to walk to the south in a similar style. To achieve such direction invariance, the current practice is to remove the facing direction's rotation around the vertical axis before further processing. Such a scheme, however, is not robust for rotational behaviors in the sagittal plane. In search of a smooth scheme to achieve direction invariance, we prove that in general a singularity free scheme does not exist. We further connect the problem with the hairy ball theorem, which is better-known to the graphics community. Due to the nonexistence of a singularity free scheme, a general solution does not exist and we propose a remedy by using a properly-chosen motion direction that can avoid singularities for specific motions at hand. We perform comparative studies using two deep-learning based methods, one builds kinematic motion representations and the other learns physics-based controls. The results show that with our robust direction invariant features, both methods can achieve better results in terms of learning speed and/or final quality. We hope this paper can not only boost performance for character animation methods, but also help related communities currently not fully aware of the direction invariance problem to achieve more robust results.

==> src/Scheme.tex <==
\section{Automatic Motion Direction Selection Algorithm}

\begin{algorithm}[h]
  \SetAlgoLined
  \KwIn{Root orientation frames $\{g_t\},~t=1, \dots, T$}
  \KwOut{The motion direction vector $r$}
 
  $n_y \leftarrow (0, 1, 0)$\;
  \For{$t \leftarrow 1$ \KwTo $T$}{
    $p_t = g^{-1}_t(n_y)$\;
   }

 
  $\{r_i\}$=UniformlySampleOnSphere($N$), $~ i = 1, \dots, N$\;
%  Denote $d_i$ as geodesic distance from $\mathbf{r}_i$ to trajectory $\{\mathbf{p}_t\}$\;
  \For{$i \leftarrow 1$ \KwTo $N$}{
    $d_i \leftarrow +\infty$\;
    \For{$t \leftarrow 1$ \KwTo $T$}{
    $d^{+}_{it}=$ComputeGeodesicDistance($r_i,p_t$)\;
    $d^{-}_{it}=$ComputeGeodesicDistance($-r_i,p_t$)\;
    $d_i = \min\{d_i,~d^{+}_{it},~d^{-}_{it}\}$\;
    }
  }
  
  $j \leftarrow \argmax_{i\in 1, \dots , N} d_i$\;
  \Return $r_j$
\caption{Motion Direction Computation}
\end{algorithm}
This algorithm is derived from the proof and derivation in Section~\ref{sec:hairy_ball} and \ref{sec:derivation}. To automatically choose the best motion direction $r$, we need to maximize the geodesic distance from $n_y$ to $g_t(r)$ and $g_t(-r)$ for the full course of the motion, which is equivalent to maximizing the geodesic distance from $g_t^{-1}(n_y)$ to $r$ and $-r$. $g_t^{-1}(n_y)$ is exactly the trajectories that we have visualized in Figure~\ref{fig:vector_field} and \ref{fig:break_dance}.

